Geometric deep learning on graphs and manifolds using mixture model CNNs

Deep learning has achieved a remarkable performance breakthrough in several fields, most notably in speech recognition, natural language processing, and computer vision. In particular, convolutional neural network (CNN) architectures currently produce state-of-the-art performance on a variety of image analysis tasks such as object detection and recognition. Most of deep learning research has so far focused on dealing with 1D, 2D, or 3D Euclidean-structured data such as acoustic signals, images, or videos. Recently, there has been an increasing interest in geometric deep learning, attempting to generalize deep learning methods to non-Euclidean structured data such as graphs and manifolds, with a variety of applications from the domains of network analysis, computational social science, or computer graphics. In this paper, we propose a unified framework allowing to generalize CNN architectures to non-Euclidean domains (graphs and manifolds) and learn local, stationary, and compositional task-specific features. We show that various non-Euclidean CNN methods previously proposed in the literature can be considered as particular instances of our framework. We test the proposed method on standard tasks from the realms of image-, graph- and 3D shape analysis and show that it consistently outperforms previous approaches.

==> CNN_graphs_manifold.tex <==
\section{CNN on Graphs and Manifold}

Defined how to construct our trainable patch operator, we can now introduce how to actually build our CNN for manifolds and graphs. It is clear that, in order to successfully apply our approach, two fundamental problems needs to be solved at first. Namely:

\begin{itemize}
\item the selection of a sufficiently good set of features capable at representing at best the structure of the domains we have to deal with.
\item the pooling operation that we may want to apply.
\end{itemize}

Because of the different nature of the problems that one may have to counter, the set of features we may need to select is unfortunately not unique, but strictly depends on the available information that describes the existing relationships between each possible pair of vertices.

In Shapes and Range scans this set may be represented by the geodesic distance and orientation existing between two considered vertices, in citation network by the degree of the nodes considered in the selected neighborhood, in Social Networks by the set of data describing the interactions between users (\eg exchanged messages, mutual likes) and so on.  
Which set of data to exploit is therefore a strictly problem dependent issue, which needs to be solved time by time, analyzing the information that may be available in the considered case. 

The same states for the pooling operation that we may decide to apply. Merging different features describing the relationships between nodes is indeed a non-trivial task and may require some domain knowledge for producing successful results. In any case we found useful to apply the Graclus algorithm as suggested in \cite{defferrard2016convolutional} for the multi-level structure it produces (which gives a comfortable way of combining different features merging just two different nodes at a time).

%\eg given geodesic distance and orientation between two nodes, after the pooling operation the features describing the relationship in the coarser graph may be equal to to the mean values of these, however this is something that may not be applied if we had for example binary features describing mutual characteristics of the vertices. 

In order to show how to apply our approach to a multitude of different situations, in the following we will deal with 3 different types of problems. Namely:

\begin{itemize}
\item Graph classification
\item Vertex classification
\item Shape correspondence
\end{itemize}

We will show how given a sufficiently good set of features, in all the above cases our approach is capable at outperforming previous solutions, while keeping at the same time a good generalization among different domains.



%Defined how to build our trainable patch operator, we can now introduce how to actually build our CNN for manifolds and graphs. It is clear that, in order to successfully apply our approach, a fundamental problem needs to be solved at first. Namely, the selection of a sufficiently good set of features capable at representing at best the structure of the domains we have to deal with. Because of the different nature of the problems that one may have to counter, this set of features is unfortunately not unique, but strictly depends on the available information that describes the existing relationships between each possible pair of vertices.
%
%In Shapes and Range scans this set may be represented by the geodesic distance and orientation existing between two considered vertices, in citation network by the degree of the nodes considered in the selected neighborhood, in Social Networks by the set of data describing the interactions between users (\eg exchanged messages, mutual likes) and so on.  
%
%Which set of data to exploit is therefore a strictly problem dependent issue, which needs to be solved time by time, analyzing the information that may be available in the considered case. In order to show how to apply our approach to a multitude of different situations, in the following we will deal with 3 different types of problems. Namely:
%
%\begin{itemize}
%\item Graph classification
%\item Vertex classification
%\item Shape correspondence
%\end{itemize}
%
%We will show how given a sufficiently good set of features, in all the above cases our approach is capable at outperforming previous approaches, keeping at the same time a good generalization  among the different domains that we will need to face.

==> results_additional_material.tex <==


\begin{figure*}[h!]
\centering
\begin{minipage}[t]{0.9\linewidth}
\includegraphics[width=1\linewidth]{./figures/CORA/GMM_prob_split_new.pdf}
\end{minipage}\vspace{2mm}
\caption{Predictions obtained applying MoNet over the Cora dataset. Marker fill color represents the predicted class; marker outline color represents the groundtruth class. }
\label{fig:cora-pred}
\end{figure*}


\input{./figures/geod_errs/max=15/geod_errs_all.tex}
\input{./figures/geod_errs_range_scans/max=15/geod_errs_range_scans_all.tex}


